SemGuard: Real-Time Semantic Evaluator for Correcting LLM-Generated Code

Large Language Models (LLMs) can translate natural language requirements into code, yet empirical analyses of representative models reveal that semantic errors-programs that compile but behave incorrectly-constitute the majority of observed faults (e.g., >60% on DeepSeek-Coder-6.7B and QwenCoder-7B). Post-hoc repair pipelines detect such faults only after execution, incurring latency, relying on incomplete test suites, and often mis-localizing the defect. Since semantic drift originates in the autoregressive decoding process, intervening while the code is being generated is a direct way to stop error propagation. Constrained-decoding approaches such as ROCODE attempt this, but still wait until the entire program runs to obtain feedback and use entropy heuristics that do not truly capture semantics. A more effective solution must inject semantic signals-early and precisely-into the decoding process.We present SemGuard, a semantic-evaluator-driven framework that performs real-time, line-level semantic supervision. To train the evaluator, we build SemDiff, the first dataset with fine-grained annotations that mark the exact line where a correct and an incorrect implementation diverge. The evaluator, once embedded in the LLM's decoder, flags deviations on partial code, rolls back to the faulty line, and guides regeneration-without executing the program or requiring test cases. Across four benchmarks, SemGuard consistently outperforms state-of-the-art baselines. It lowers the semantic error rate by 19.86% on SemDiff relative to ROCODE, and lifts Pass@1 by 48.92% on the real-world LiveCodeBench with CodeLlama-7B. Similar gains hold for StarCoder2-7B on MBPP and for DeepSeekCoder-6.7B on the Java benchmark SemDiff-Java, demonstrating model- and language-agnostic effectiveness.

==> tables/04.tex <==
% \begin{table}[!t]
%   \flushleft
%   \caption{The generalization capability of SemGuard in LivecodeBench.}
%   % 如已在导言区设置 \arraystretch，可去掉下一行
%   \renewcommand{\arraystretch}{1.3}
%   % 按当前栏宽的80%等比放大
%   \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{lccc}  % 无竖线
%       \toprule           % 第一条横线（表头上方）
%       \makecell{\textbf{Model}}
%         & \makecell{\textbf{Temperature}\\\textbf{Sampling}}
%         & \makecell{\textbf{SemGuard}\\\textbf{random}}
%         & \makecell{\textbf{SemGuard}\\\textbf{penal}} \\
%       \midrule           % 第二条横线（表头下方）
%       DeepseekCoder-6.7B &  7.68 &  8.75 & \textbf{10.04} \\
%       QwenCoder-7B       &  8.62 &  9.57 & \textbf{10.87} \\
%       StarCoder2-7B      &  6.74 &  7.20 &  \textbf{8.74} \\
%       CodeLlama-7B       &  5.56 &  7.09 &  \textbf{8.28} \\
%       \bottomrule        % 第三条横线（表尾下方）
%     \end{tabular}%
%   }

%   \label{tab:table-livecodebench}
% \end{table}


\begin{table}[!t]
  \flushleft
  \caption{The generalization capability of SemGuard in LivecodeBench.}
  % 如已在导言区设置 \arraystretch，可去掉下一行
  \renewcommand{\arraystretch}{1.3}
  % 按当前栏宽的80%等比放大
  \resizebox{\columnwidth}{!}{%
  \renewcommand{\arraystretch}{1.5} % 调整行距，1.5倍行距
    \begin{tabular}{l|ccc}  % 无竖线
      \toprule           % 第一条横线（表头上方）
      \makecell{\textbf{Model}}
        & \makecell{\textbf{Temperature}\\\textbf{Sampling}}
        & \makecell{\textbf{SemGuard}\\\textbf{random}}
        & \makecell{\textbf{SemGuard}\\\textbf{penal}} \\
      \midrule           % 第二条横线（表头下方）
      DeepseekCoder-6.7B &  7.68 &  \coloryellow8.75 & \colorblue \textbf{10.04} \\
      QwenCoder-7B       &  8.62 &  \coloryellow9.57 & \colorblue \textbf{10.87} \\
      StarCoder2-7B      &  6.74 &  \coloryellow7.20 & \colorblue \textbf{8.74} \\
      CodeLlama-7B       &  5.56 &  \coloryellow7.09 & \colorblue \textbf{8.28} \\
      \bottomrule        % 第三条横线（表尾下方）
    \end{tabular}%
  }

  \label{tab:table-livecodebench}
\end{table}
